Absolutely continuous spectrum for a random potential on a tree with strong transverse correlations and large weighted loops

We consider random Schr\"odinger operators on tree graphs and prove absolutely continuous spectrum at small disorder for two models. The first model is the usual binary tree with certain strongly correlated random potentials. These potentials are of interest since for complete correlation they exhibit localization at all disorders. In the second model we change the tree graph by adding all possible edges to the graph inside each sphere, with weights proportional to the number of points in the sphere.

==> discards.tex <==
Repeating this procedure $N$ times results in the formula
$$\displaylines{\quad
M_{a,\alpha,\lambda}= \int_\HH\int_{\RR^2}\cdots \int_{\RR^2}\chi(u)\; \chi(\phi_{\qq_1,\lambda}(u))\cdots
\chi(\phi_{\qq_1,\lambda}\circ \phi_{\qq_2,\lambda}\circ \cdots \circ \phi_{\qq_N,\lambda}(u))\;
\hfill\cr\hfill
\cd(\phi_{\qq_1,\lambda}\circ \phi_{\qq_2,\lambda}\circ \cdots \circ \phi_{\qq_N,\lambda}(u))^{1+\alpha}\;d\nu_a(\qq_1)d\nu_a(\qq_2)\cdots d\nu_a(\qq_N)\;d\rho_{a,\lambda}(u) + C.
\quad}$$

Define

Then we can rewrite the formula above as
$$
M_{a,\alpha,\lambda}= \int_\HH m_{a,\alpha,\lambda}(u) \cd(u)^{1+\alpha} d\rho_{a,\lambda}(u)
$$
where
$$\displaylines{\quad
m_{a,\alpha,\lambda}(u) = \int_{\RR^2}\cdots \int_{\RR^2}
\chi(u) \mu_{\qq_1,\lambda}^{1+\alpha}(u)
\;\;\;
\chi(\phi_{\qq_1,\lambda}(u)) \mu_{\qq_2,\lambda}^{1+\alpha}(\phi_{\qq_1,\lambda}(u))\cdots
\hfill\cr\hfill
\cdots\chi(\phi_{\qq_1,\lambda}\circ \cdots \circ \phi_{\qq_{N-1},\lambda}(u)) \mu_{\qq_N,\lambda}^{1+\alpha}(\phi_{\qq_1,\lambda}\circ \cdots \circ \phi_{\qq_{N-1},\lambda}(u))
\lastdisplayline{mdef}{\hfill\cr\hfill
\chi(\phi_{\qq_1,\lambda}\circ \cdots \circ \phi_{\qq_{N},\lambda}(u))d\nu_a(\qq_1) \cdots d\nu_a(\qq_N)
\quad}}$$
If we can bound
$$
m_{a,\alpha,\lambda}(u) \le 1-\epsilon_1
$$
uniformly for $u\in\HH$, $|\Re(\lambda)| \le \lambda_0$ and $0\le\lambda\le\epsilon$ we are done, since in that
case
$$
M_{a,\alpha,\lambda} \le (1-\epsilon_1)M_{a,\alpha,\lambda} + C
$$
uniformly for $|\Re(\lambda)| \le \lambda_0$ and $0\le\lambda\le\epsilon$. Then
$$
\sup_{{|\Re\lambda|\le\lambda_0}\atop{0<\Im\lambda\le\epsilon}} M_{a,\alpha,\lambda} \le C/\epsilon_1
$$
and we can invoke \thmrf{Mimplies}

To procede we introduce an averaged version of $\mu$ 

and estimate 
$$
m_{a,\alpha,\lambda}(u) \le \sup_\qq \chi(\phi_{\qq,\lambda}(u))\overline\mu_{a,\alpha,\lambda}(\phi_{\qq,\lambda}(u))\;\; \chi(u)\overline\mu_{a,\alpha,\lambda}(u)
$$
Here we used \rf{mdef} with $N=2$. The supremum over $\qq$ is taken over the support of $d\nu_a$, that is, $|q_1|\le a$ and
$|q_2|\le a$. To use this formula we need the following estimate on $\overline\mu$. This is the main technical result in 
this part of the paper. 

\beginlemma

\endlemma


==> extensions.tex <==
\hd{5. Extensions and open problems}

For $\delta = 0$, that is, when the random variables $q_1$ and $q_2$ are independent, our result gives
$\lambda_0 = 2$. An obvious question is ``How large can $\lambda_0$ actually be?''. When $\lambda_0$ is  larger than $2$ the polynomial $p(u,\lambda,\delta)$ in \rf{mubarbdd} changes sign so the estimate for
$\overline\mu_{a,\alpha,\lambda}(u)$ goes above $1$ for some values of $u$. However, the product on the right side of 
\rf{obv} remains bounded below $1$ if $\lambda_0$ is only slightly larger than $2$, since the second term in the product compensates. So, our proof can accommodate $\lambda_0$ slightly larger than $2$. To push $\lambda_0$ even higher, we can consider iterating the procedure leading to \rf{Mbdd2} an arbitrary number of times. This would presumably allow even
larger values of $\lambda_0$ at the expense of more complicated proofs. The determination of the exact range of absolutely continuous spectrum (as indeed the question of band-edge localization for this model) remains open. 

At first glance, it appears that the assumption that the distributions $\nu_a$ are identical for each sphere seems essential. Dropping it means that we lose self-similarity in the tree. However, in fact it is possible to handle the case where the distribution for the $n$th sphere $\nu_{a,n}$ can depend on $n$, provided that each distribution satisfies the assumptions \rf{nuassn1}, \rf{nuassn3} and \rf{nuassn2}. Then the distributions $\rho_{a,\lambda,n}$ and the moments $M_{a,\alpha,\lambda,n}$ also vary from sphere to sphere. 
In this setup we are interested in $M_{a,\alpha,\lambda,1}$.
The methods in this paper (with two iterations) can then be used to show that for suitable $a$, $\alpha$ and $\lambda$ 
\be{ndep}
M_{\lambda,n} \le (1-\epsilon)M_{\lambda,n+2} + C.
\ee
(We have dropped the $a$ and $\alpha$ subscripts.) Here $\epsilon$ and $C$ are positive constants that are independent of $n$ and $\lambda$. Iterating this bound $N$ times gives
$$\eqalign{
M_{\lambda,1} &\le (1-\epsilon)^NM_{\lambda,1+2N} + C\left(\sum_{k=1}^{N-1}(1-\epsilon)^k\right)\cr
&\le (1-\epsilon)^NM_{\lambda,1+2N} + {{C}\over{\epsilon}}.\cr
}$$
This estimate may appear useless, but for $\Im(\lambda) > 0$ we actually have an $n$ independent (but $\lambda$ dependent!) bound on  $M_{\lambda,n}$, because the support of $\rho_{a,\lambda,n}$ is contained in a $\lambda$ dependent 
compact set. Hence we obtain
$$
M_{\lambda,1} \le (1-\epsilon)^N C_\lambda + {{C}\over{\epsilon}}
$$
and we may send $N\rarr \infty$ to obtain the desired bound on $M_{\lambda,1}$.


==> intro.tex <==
\hd{Abstract}
We consider random Schr\"odinger operators on tree graphs and
prove absolutely continuous spectrum at small disorder for two models. 
The first
model is the usual binary tree with certain strongly
correlated random potentials. These potentials are of interest since for
complete correlation they exhibit localization at all disorders. In the second model 
we change the tree graph by adding all possible edges to the graph inside each sphere,
with weights proportional to the number of points in the sphere.

\bigskip
Mathematics subject classification number: 82B44




\hd{1. Introduction}

Proving the existence of absolutely continuous spectrum for random 
Schr\"odinger operators at weak disorder remains a challenging problem.
The extended states conjecture, asserting the existence of
absolutely continuous spectrum at low disorder for the Anderson model on $\ZZ^d$, $d\ge 3$
remains the most important open problem in the field. 
When $\ZZ^d$ is replaced by the Bethe Lattice (or tree graph)
this conjecture has been proved by Klein [K], extended and reproved by Aizenman, Sims and Warzel [ASW],
and given yet another proof by the present authors [FHS2]. Our proof, which only applied to binary trees, 
has been simplified and 
extended by Halasan [H] to
cover trees with higher branching number, and with additional vertices. (See also Spitzer [Sp].) Recent work on spectral theory for
discrete Schr\"odinger operators on trees includes Breuer [B1] and [B2] and Breuer and Frank [BF].

There is a large gap between the known results for the tree and the open problem on $\ZZ^d$.
This present paper is an attempt to address some of the problems that would come up on $\ZZ^d$ in 
 simpler models.
The paper has two parts. In the first part we consider a binary tree
with a transversely 2-periodic random potential. The potential is defined by choosing two values
of the potential at random, independently for each sphere or level (that is, a set of vertices 
a fixed distance in the graph from the origin) in the tree. These two 
values are then repeated periodically across the sphere. The point of this model is that although the underlying
graph is still a tree, we have negated some of the advantage of the exponential spreading of the tree.

In fact, such two-periodic potentials can exhibit either dense 
point spectrum or absolutely continuous spectrum.
In our previous paper [FHS1], the values
$(q_1,q_2)$ were chosen close to $(\delta,-\delta)$ for $\delta > 0$. In this case
we obtained a deterministic result proving existence of absolutely continuous spectrum.
On the other hand, if $(q_1,q_2)$ are chosen randomly on the diagonal $q_1=q_2$ then the potential is radial, 
and this model is equivalent to a one-dimensional Anderson model that exhibits localization at all disorders. 

We will prove that if the potentials $(q_1,q_2)$ are sufficiently uncorrelated (see assumption \rf{nuassn2} below) then there will be some absolutely 
continuous spectrum, as is the case for the Anderson model.
However, since in some sense this model is so close to being one-dimensional, the proof
has some features not appearing in [FHS2]. 
In both [FHS2] and the present paper, the proofs follow from an 
estimate of an average over potential values $q$ of functions
$\mu(z,q)$, similar in both models, that measure the contraction of a relevant map of
the plane. We seek an estimate of the form $\int \mu(z,q) d\nu(q) < 1$ for $z$ near the boundary at infinity.
In [FHS2] we use the independence of the potentials across the sphere in proving that
$\mu(z,0)$ is already less than one. Then small values of $q$ in the integral are handled by semi-continuity. 
In the present
situation $\mu(z,q)$ for $q=0$ is identically equal to one, and perturbations
in $q$ send it in both directions. Thus we must use cancellations in the integral
over $q$ in an essential way. 

Our method extends to the case where the joint distributions are not identical, as long
as they are all centered and satisfy certain uniform bounds.
This is significant since in this case we lose the self-similarity that has been used in previous proofs.  

Another obvious way that $\ZZ^d$  differs from the tree is in the presence
of arbitrarily large loops. In the second part of this paper, we show how to introduce (weighted)
loops with unbounded size into the model from the first part. We introduce connections between 
every pair of vertices in a given sphere, weighted to make the total weight
of the added edges equal to one in each sphere. This is a sort of mean-field
interaction. These connections mean that when we remove the interior of some ball from the 
graph, the resulting exterior domain does not consist of disconnected pieces equivalent
to the original graph, as is the case for the tree.
Nevertheless, we can prove absolutely continuous spectrum for this model using
results from the first part of this paper in a two-step procedure. To reduce the technical 
complication, we will only consider a Bernoulli distribution for the potentials in this section.

In the next section we review the basic set-up for calculating a diagonal matrix
element of the Green's function for discrete random 
Schr\"odinger operators, using a decomposition of the graph and the
corresponding sequence of forward Green's functions. In Section 3 we specialize to a tree model with
a strongly transversely correlated random potential and present \thmrf{twoperiodic}, the first main
theorem. The bounds on the moment required in the proof of this theorem
are given in Section 4 but the proof of the main technical \thmrf{mubarbdd} is
postponed to Section 6. Section 5 deals with extensions and open
problems related to our method of proof. The last two sections are
devoted to the mean-field tree model. \thmrf{meanfield} is our second main result. 
A proof of the main technical \thmrf{finalbdd} needed for this theorem is relegated to
Section 8. 


\hd{2. Review of basic setup}

Let $(V,E)$ be a graph with vertex set $V$ and edges $E \subseteq V\times V$, and
let $\gamma:E\rarr \RR^+$ be a bounded symmetric function. Let $L$ be the Laplacian 
with matrix elements given by
$$
L_{v,w} =\cases{
\displaystyle{\gamma ((v,w))} & if $(v,w)\in E$ \cr\cr
0 & otherwise\cr
}.
$$
We assume that the number of edges joining a vertex is uniformly bounded. Then $L$ is a bounded,
self-adjoint operator on $\ell^2(V)$.

Given a potential $q:V\rarr\RR$, let $Q$ be the operator of multiplication by $q$
with matrix elements $Q_{v,w} = q(v) \delta_{v,w}$.
We are interested in the spectrum of the discrete Schr\"odinger operator 
$$
H=L+Q
$$ acting
in $\ell^2(V)$. Let $0\in V$ denote a distinguished vertex. We will study the spectral measure for $H$ for the vector $\delta_0 \in \ell^2(V)$ given by
$$
\delta_0(v) = \cases{ 1 & if $v=0$\cr 0 & otherwise\cr}
$$
through its Borel transform given by the Green's function
$G_0(\lambda) = \jap{\delta_0, (H-\lambda)^{-1} \delta_0}$.

Our approach is based on a decomposition of $V$ as a disjoint union
and the corresponding direct sum decomposition of $\ell^2(V)$
$$
V = \bigcup_{n=0}^\infty S_n, \quad \ell^2(V) = \bigoplus_{n=0}^\infty \ell^2(S_n).
$$
We assume that $S_0 = \{0\}$ and that vertices in $S_n$ are only connected to vertices
in $S_{n-1}$, $S_{n}$ and $S_{n+1}$. (We will take take the sets $S_n$ to be spheres containing
all vertices a distance $n$ in the graph from $0$.)
Then the block matrix forms of 
$L$ and $H$ have zeros away from the diagonal and first off-diagonal blocks.
$$
L = 
\left[\matrix{
D_0 	&E_0^T 	&0 	&0 	& \cdots \cr
E_0 	&D_1	&E_1^T	&0	& \cdots \cr
0	&E_1	&D_2	&E_2^T	& \cdots \cr
\vdots	&\vdots	&\vdots	&\vdots	& \ddots \cr
}\right],
\quad
H = 
\left[\matrix{
D_0+Q_0	&E_0^T 	&0 	&0 	& \cdots \cr
E_0 	&D_1+Q_1	&E_1^T	&0	& \cdots \cr
0	&E_1	&D_2+Q_2	&E_2^T	& \cdots \cr
\vdots	&\vdots	&\vdots	&\vdots	& \ddots \cr
}\right].
$$
According to the formula for $L$, the matrix $D_n$ is the Laplacian for the sphere $S_n$, while $E_n$
has non-zero entries corresponding to the connections between $S_n$ and $S_{n+1}$.
Let $P_n$ denote the projection of $\ell^2(V)$ onto $\ell^2(S_n)$ and define
$P_{n,\infty} = \sum_{k=n}^\infty P_n$. Define
$H_n = P_{n,\infty}\,H\,P_{n,\infty}$
and the forward Green's functions
$$
G_n(\lambda) = P_n (H_n-\lambda)^{-1} P_n.
$$
Each $G_n(\lambda)$ is a $d_n\times d_n$ matrix, where $d_n$ is the number of vertices in $S_n$
and lies in the Siegel upper half space $\SH_{d_n}$, that is, the space of symmetric $d_n\times d_n$ matrices with positive definite imaginary part. Note that $\SH_1=\HH$ is the usual upper half plane of $\CC$.

The forward Green's functions are related by the formula
\be{recursion}
G_n(\lambda) = \Phi_n(G_{n+1}, Q_n, \lambda),
\ee
where $\Phi_n:\SH_{d_{n+1}}\times S_{d_n}\times\HH \rarr \SH_{d_n}$ is given by
$$
\Phi_n(G_{n+1}, Q_n,\lambda)=-\left(E_n^TG_{n+1}E_n-D_n-Q_n+\lambda\right)^{-1}.
$$
Here $S_d$ is the set of $d\times d$ real symmetric matrices.
To see this, note that
$G_n(\lambda)$ is the top left corner block of
$$
\left[\matrix{
D_n+Q_n-\lambda	&\matrix{E_n^T 	&0 	&0 	& \cdots \cr}\cr
\matrix{E_n\cr 0\cr \vdots \cr} & H_{n+1}-\lambda \cr
}\right]^{-1}.
$$
Thus, according to 
Schur's formula 
\be{schur}
\twomat{A & B^T}{B & C}^{-1} = \twomat{(A-B^TC^{-1}B)^{-1} & (BC^{-1}B^T-A)^{-1}BC^{-1}}{C^{-1}B^T(BC^{-1}B^T-A)^{-1} & (C-B^TA^{-1}B)^{-1}}
\ee
for the inverse of a symmetric block matrix we have
$$\eqalign{
G_n(\lambda) &= -\left(\left[\matrix{E_n^T 	&0 	&0 	& \cdots \cr}\right]
(H_{n+1}-\lambda)^{-1}\left[\matrix{E_n\cr 0\cr \vdots \cr}\right]-D_n-Q_n+\lambda\right)^{-1},\cr
}$$
which implies \rf{recursion}.

Now suppose that the potential is chosen at random, independently for every sphere $S_n$ 
according to a probability distribution $N_n$ on $\RR^{d_n}$. Then the matrices $G_n(\lambda)$ are
random variables, distributed according to some measure $R_{n,\lambda}$ on $\SH_{d_n}$, 
and \rf{recursion} implies that $R_{n,\lambda}$ is the push-forward of $R_{n+1,\lambda}\times N_n$
under $\Phi_n$. This means that for every integrable function $f$ on $\SH_{d_n}$
\be{probrecursion}
\int_{\SH_{d_n}} f(Z)\, dR_{n,\lambda}(Z) = \int_{\SH_{d_{n+1}}}\int_{\RR^{d_n}} f(\Phi_n(Z,Q,\lambda))\, dN_n(Q)\, dR_{n+1,\lambda}(Z).
\ee

The measure in which we really are interested is $R_{0,\lambda}$, the distribution for $G_0$, which is a 
probability measure on $\HH$. In our examples, we will use formula \rf{probrecursion} 
to prove a bound of the form
\be{moment}
\sup_{{|\Re(\lambda)| \le \lambda_0}\atop{0<\Im(\lambda)\le \epsilon}} \int_\HH w(z)^{1+\alpha} dR_{0,\lambda}(z)
< \infty,
\ee
where $\alpha > 0$ and $w(z)$ is a weight function satisfying
\be{wtassn}
\Im(z) \le C w(z)
\ee
for $z$ in a neighbourhood of the boundary at infinity $\PA_\infty \HH$. In the upper half plane model of hyperbolic space $\HH$, the boundary at infinity is $\RR \cup \{i\infty\}$. A neighbourhood of $\PA_\infty \HH$ is the complement of a closed bounded set in $\HH \cup \PA_\infty \HH$. 
Here and throughout the paper, $C$ denotes a generic constant that may change from line to line.
Notice that the integral in formula \rf{moment} is the expectation ${\Bbb E}\left[\cd(G_0(\lambda))^{1+\alpha}\right]$.

\beginlemmalabel{KS}
Suppose that \rf{moment} holds for some $\alpha>0$ and some weight function $w$ satisfying
\rf{wtassn}.
Then the spectral measure $\mu_0$ of which $G_0(\lambda)$ is the Borel transform is almost surely 
purely absolutely continuous in $(-\lambda_0,\lambda_0)$.
\endlemmalabel
\beginproof (Following Klein [K] and Simon [Si].) By Fatou's Lemma and \rf{moment}
$$
\Bbb E\left(
\liminf_{\epsilon \downarrow 0} \int_{-\lambda_0}^{\lambda_0} w(G_0(x+i\epsilon))^{1+\alpha} dx
\right)
\le 
\liminf_{\epsilon \downarrow 0}\int_{-\lambda_0}^{\lambda_0} \Bbb E\left(w(G_0(x+i\epsilon))^{1+\alpha}\right) dx < C.
$$
This implies that for almost every choice of potential
$$
\liminf_{\epsilon \downarrow 0} \int_{-\lambda_0}^{\lambda_0} \left(\Im(G_0(x+i\epsilon))\right)^{1+\alpha} dx
\le C \liminf_{\epsilon \downarrow 0} \int_{-\lambda_0}^{\lambda_0} w(G_0(x+i\epsilon))^{1+\alpha} dx
<C.
$$
So, for such a potential, there exists a sequence $\epsilon_n \downarrow 0$ such that 
$$
\sup_n\int_{-\lambda_0}^{\lambda_0} \left(\Im(G_0(x+i\epsilon_n))\right)^{1+\alpha} dx < C.
$$
Then, since $\pi^{-1}\Im G_0(x+i\epsilon) dx$ converges to $d\mu_0(x)$ weakly (see [Si]) as $\epsilon\downarrow 0$ 
we find that for any compactly supported continuous function $f$
$$\eqalign{
\left|\int_{-\lambda_0}^{\lambda_0} f(x) d\mu_0(x)\right|
&= \lim_{n\rarr\infty} \pi^{-1}\left|\int_{-\lambda_0}^{\lambda_0} f(x)\Im G_0(x+i\epsilon_n) dx \right|\cr
&\le \limsup_{n\rarr\infty} \pi^{-1}\left[\int_{-\lambda_0}^{\lambda_0} |f(x)|^q dx\right]^{1/q}
\left[\int_{-\lambda_0}^{\lambda_0} \left(\Im G_0(x+i\epsilon_n)\right)^{1+\alpha} dx\right]^{1/(1+\alpha)}\cr
&\le C\|f\|_q. \cr
}$$
Here $q$ is the dual exponent to $1+\alpha$ in H\"older's inequality. This implies that $d\mu_0(x) = g(x) dx$ for some $g\in L^{1+\alpha}$ and completes the proof.
\endproof


==> meanfield.tex <==
\hd{7. A mean-field model}

In this section we add a weighted complete graph to every sphere in the tree. Since the weights are chosen to make the total added weights the same in each sphere, this is a sort of mean-field model. Pick a number $\gamma >0$. Each added
edge (dotted line in the diagram below) in the $n$th sphere $S_n$ is given the weight $\gamma 2^{-n}$.
\vskip 20pt
\epsfxsize=4cm
\centerline{\epsffile{mf.eps}}
We call this graph the mean-field binary tree. The spectrum of the free Laplacian on the mean-field tree is
the union of two intervals $[-2\sqrt{2}+\gamma,2\sqrt{2}+\gamma]\cup[-2\sqrt{2},2\sqrt{2}]$ and is
purely absolutely continuous. This can be seen by diagonalizing the Laplacian using a Haar basis, as in [AF].


To simplify the calculations, we will consider this model when the transversely two-periodic potential 
is defined by the product of two independent Bernoulli distributions for $q_1$ and $q_2$,
$$
\nu = {{1}\over{4}}\big(\delta(q_1-1) + \delta(q_1+1)\big)\big(\delta(q_2-1) + \delta(q_2+1)\big).
$$

\begintheoremlabel{meanfield}
Let $\nu$ be the product of Bernoulli distributions defined above and
let $H_{a,\gamma}$ be the random discrete Schr\"odinger operator on the mean-field binary tree corresponding to the transversely two-periodic potential defined by the scaled distribution $\nu_a$ and weight $\gamma$. There exist $0 < \lambda_0, \lambda_1 < 2\sqrt{2}$ such that for sufficiently small $a$ the spectral measure for $H_a$ corresponding to $\delta_0$ has purely absolutely continuous spectrum in $\{\lambda: |\lambda|\le \lambda_0,|\lambda - \gamma|\le\lambda_1\}$.
\endtheoremlabel

In this theorem, the constant $\lambda_0$ has the same value as in the first part of the paper, while
$\lambda_1$ can be taken to be any positive number less that $2\sqrt{2}$.

The forward Green's functions $G_n$ are not diagonal. In the basic recursion formula \rf{recursion} for the forward Green's functions on the mean-field tree the matrices $E_n$ and $Q_n$ are unchanged from the binary tree, but the matrices $D_n$ are now $2^{-n}\gamma$ times the Laplace operator for the complete graph on $S_n$. This Laplace operator is a $2^n\times 2^n$ matrix with each diagonal entry equal to zero and each off-diagonal entry equal to $1$. Thus 
$$
D_n = \gamma (P - 2^{-n}I),
$$
where $P$ projects onto $2^{-n/2}[1,1,\ldots,1]^T$. Introduce the $d_n\times d_n$ matrix 
$$
U_n = E_n^TG_{n+1}E_n - D_n + \lambda = E_n^TG_{n+1}E_n -\gamma P +\lambda_n,
$$
where
\be{lambdan}
\lambda_n = \lambda + \gamma 2^{-n}.
\ee
Then the basic recursion formula reads
$$
U_{n-1} = -E_{n-1}^T (U_n - Q_n)^{-1} E_{n-1} - \gamma P + \lambda_{n-1}.
$$



The range of $P$ is the span of the first vector in the Haar basis. Since the representation of a two-periodic potential in this basis is not too complicated, it is natural to change to this basis
to simplify the problem. Here is a diagram of the Haar basis for $\ell^2(S^n)=\CC^{2^n}$ with $n=3$. Each vector is normalized to make the basis orthonormal.
This basis has a natural tree structure determined by the supports of the vectors. The highest level is the constant vector,
and the lowest level consists of vectors with two non-zero entries of $\pm 2^{-1/2}$.
\vskip 20pt
\epsfxsize=8cm
\centerline{\epsffile{haar.eps}}
\vskip 20pt

Let $V_n$ be the $2^n\times 2^n$ orthogonal change of basis matrix to the Haar basis, whose columns consist of the Haar basis vectors.
\beginlemmalabel{Vstuff}\par
(i) $V_n^T P V_n = \diag[1,0,0,\ldots]$.\par
(ii) $V_n^T E_n^T V_{n+1} = \sqrt{2}[I,{\bf 0}]$.\par
(iii) Let $Q=\diag[q_1,q_2,q_1,q_2,\ldots]$ be a two-periodic potential. Setting $\bar q = (q_1+q_2)/2$ and $\tilde q = (q_1-q_2)/2$ we have
$$
V_n^T Q V_n = \bar q I + \tilde q \twomat{{\bf 0} & V_{n-1}^T}{V_{n-1} & {\bf 0}}.
$$
\par
\endlemma
The proof of this lemma is a straightforward computation, which we omit. Now we write the matrix $U_n$ in the Haar basis.
Define
$$
\tilde U_n = V_n^TU_nV_n.
$$
In view of \thmrf{Vstuff}, the recursion formula for $\tilde U_n$ reads
\be{utilderecursion}
\tilde U_{n-1} = -2[I,{\bf 0}]\left(
\tilde U_n  - \bar q - \tilde q\twomat{{\bf 0}& V_{n-1}^T}{V_{n-1}&{\bf 0}}
\right)^{-1} \twomat{I}{\bf 0} -\gamma \diag[1,0,0,\ldots]  + \lambda_{n-1},
\ee
where $\lambda_n$ is given by \rf{lambdan}.
This recursion formula preserves matrices of the form $\diag[u_1,u_2,u_2,\ldots]$.
\beginlemma
Suppose that $\tilde U_n = \diag[u_1,u_2,u_2,\ldots]$. Then $\tilde U_{n-1}$, defined by the recursion formula
above, has the form
$$
\tilde U_{n-1} = \diag[\psi_{\qq,\lambda,\gamma,n-1}(u_1,u_2),\phi_{\qq,\lambda,n-1}(u_2),\phi_{\qq,\lambda,n-1}(u_2),\ldots],
$$
where
\be{psiphidef}\eqalign{
\psi_{\qq,\lambda,\gamma,n}(u_1,u_2) &= -{{2}\over{u_1 -\bar q - \tilde q^2(u_2-\bar q)^{-1}}} + \lambda_n -\gamma, \cr
\phi_{\qq,\lambda,n}(u_2) &= -{{2}\over{u_2-\bar q - \tilde q^2(u_2-\bar q)^{-1}}} + \lambda_n,\cr
}\ee
and $\lambda_n$ is given by \rf{lambdan}.
\endlemma
\beginproof
We have
$$
\left(
\tilde U_n  - \bar q - \tilde q\twomat{{\bf 0}& V_{n-1}^T}{V_{n-1}&{\bf 0}}
\right)^{-1}
=\twomat{A&B^T}{B&C},
$$
where
$$\eqalign{
A &= \diag[u_1 -\bar q, u_2-\bar q, u_2-\bar q,\ldots],\cr
B &= -\tilde q V_{n-1},\cr
C &= (u_2-\bar q) I.\cr
}$$
The top left block of this inverse is given by Schur's formula $(A-B^TC^{-1}B)^{-1}$. 
Since $B^TC^{-1}B = \tilde q^2 (u_2-\bar q)^{-1}V_{n-1}^TV_{n-1} = \tilde q^2 (u_2-\bar q)^{-1}I$,
the result is a diagonal matrix with $\big(u_1 -\bar q - \tilde q^2(u_2-\bar q)^{-1}\big)^{-1}$ in
the upper left corner and $\big(u_2-\bar q - \tilde q^2(u_2-\bar q)^{-1}\big)^{-1}$ in the other diagonal
positions.
The recursion formula picks out this block, multiplies by $-2$
and then adds $-\gamma \diag[1,0,0,\ldots] + \lambda_{n-1}$. This gives the formulas \rf{psiphidef}.
\endproof

The fact that the recursion formula for $\tilde U_n$ preserves diagonal matrices having the form $\diag[u_1,u_2,u_2,\ldots]$ means that $\tilde U_n$ must actually have this form. This follows from the limit formula for the forward Green's functions proved in [FHS1] which implies that these matrices will lie in any set that is preserved by the recursion flow. 
Thus, there are two random variables $u_1$ and $u_2$ for each sphere that describe the forward Green's function.
For the $n$th sphere, they are distributed according to some joint measure $\rho_{a,\lambda,\gamma,n}$ for $(u_1,u_2)$. 
Since the variables for adjacent spheres are related by \rf{psiphidef} the recursion formula for these measures reads
$$\displaylines{\quad
\int_{\HH\times\HH}w(u_1,u_2) d\rho_{a,\lambda,\gamma,n}(u_1,u_2)
\hfill\cr\hfill
= \int_{\HH\times\HH} \int_{\RR^2}
w(\psi_{\qq,\lambda,\gamma,n}(u_1,u_2),\phi_{\qq,\lambda,n}(u_2)) \,d\nu_a(\qq) \,d\rho_{a,\lambda,\gamma,n+1}(u_1,u_2).
\quad}$$

Define the moments
$$
M_{a,\alpha,\lambda,\gamma,n} = \int_{\HH\times\HH} \cd_{1,n}(u_1)^{1+\alpha} d\rho_{a,\lambda,\gamma,n}(u_1,u_2),
$$
where
$$
\cd_{1,n}(u_1) = {{|u_1-u_{\lambda_n-\gamma}|^2}\over{\Im(u_1)}}.
$$
Our goal is to bound $M_{a,\alpha,\lambda,\gamma,0}$ for $a$ and $\alpha$ small and $\lambda$ and $\gamma$ in some range. When $n=0$ then $\tilde U_0 = U_0 = [u_1] = E_0^TG_1E_0 + \lambda$.
Since $G_0 = -(E_0^TG_1E_0 + \lambda -q_0)^{-1}$ we can use the argument of \thmrf{Mimplies} to prove the existence of absolutely
continuous spectrum from such a bound.

Observe now that the recursion for $u_2$ is the same as the formula for $u$ in the first part of the paper, except that
$\lambda$ is replaced by $\lambda_{n}$. Explicitly,
$$
\phi_{\qq,\lambda_{n}}(u) = \phi_{\qq,\lambda,n}(u),
$$
where the $\phi$ is given on the left by \rf{phidef} and on the right by \rf{psiphidef}.
We claim this implies that
\be{M2bdd}
M^{(2)}_{a,\alpha,\lambda,\gamma,n} = \int_{\HH\times\HH} \cd_{2,n}(u_2)^{1+\alpha} d\rho_{a,\lambda,\gamma,n}(u_1,u_2) \le C,
\ee
provided $|\lambda| < \lambda_0$. Here
$$
\cd_{2,n}(u_2) = {{|u_2-u_{\lambda_n}|_+^2}\over{\Im(u_2)}}.
$$
The function $|z|_+$ is equal to $|z|$ except near $z=0$ where it has been modified to be
bounded away from zero. This makes no difference to the growth properties, but will allow us
to make a needed lower bound in the next section.
For large $n$ the bound \rf{M2bdd} follows from the results in the first part of the paper (extended to 
distributions that vary from sphere to sphere) since the small perturbations $\gamma 2^{-n}$ of $\lambda$ are easily
absorbed in the proof. The result for 
large $n$ suffices, since it is easy to iterate the bound \rf{M2bdd} a finite number of steps. All that is required
is an upper bound $\mu_{\qq,\lambda_{n}}(u) \le C$, for $\mu$ given by \rf{mudef}.

Similarly, it is enough to bound $M_{a,\alpha,\lambda,\gamma,n}$ for large $n$. We follow the same basic steps as before to begin the proof of such a bound. Then, one iteration gives 
%\mcomment{put in the domains of integration}
$$\displaylines{\quad
M_{a,\alpha,\lambda,\gamma,n} 
\hfill\cr\hfill
\eqalign{
&=\int_{\HH\times\HH} \cd_{1,n}(u_1)^{1+\alpha} d\rho_{a,\lambda,\gamma,n}(u_1,u_2)\cr
&= \int_{\HH\times\HH} \int_{\RR^2} \cd_{1,n}(\psi_{{\qq,\lambda,\gamma,n}}(u_1,u_2))^{1+\alpha} d\nu_a(\qq) d\rho_{a,\lambda,\gamma,n+1}(u_1,u_2)\cr
&= \int_{\HH\times\HH} \int_{\RR^2} \big(\cd_{1,n}(\psi_{{\qq,\lambda,\gamma,n}}(u_1,u_2)) - C_1 \cd_{2,n}(u_2) + C_1 \cd_{2,n}(u_2)\big)^{1+\alpha} \cr
&\quad\quad \cdot  d\nu_a(\qq) d\rho_{a,\lambda,\gamma,n+1}(u_1,u_2)\cr
&\le \int_{\HH\times\HH} \int_{\RR^2} 2^\alpha \Big[\cd_{1,n}(\psi_{{\qq,\lambda,\gamma,n}}(u_1,u_2)) - C_1 \cd_{2,n}(u_2)\Big]_+^{1+\alpha}  d\nu_a(\qq) d\rho_{a,\lambda,\gamma,n+1}(u_1,u_2)\cr
&\quad\quad + 2^\alpha C_1^{1+\alpha} M^{(2)}_{a,\alpha,\lambda,\gamma,n}.\cr
}
\quad}$$
The notation $[x]_+$ denotes $\max\{0,x\}$, not to be confused with $|z|_+$.
Here we used the convexity of $x\mapsto x^{1+\alpha}$. The positive constant $C_1$ can be chosen as large as we please.

Let $\chi(u_1)$ be a cutoff with support where $u_1$ is in a neighbourhood of $\PA_\infty\HH$. We wish to insert
this cutoff to the right of $\Big[\cdots\Big]_+^{1+\alpha}$ at the price of an overall constant. 
To do this we must show that
the quantity inside the brackets is bounded from above as $u_1$ ranges through the support of $1-\chi$.
Since $\nu_a$ is a product of Bernoulli measures there are only four possible values for $\qq$, namely
$\qq=(\pm a, \pm a)$, to
consider, and it is enough to demonstrate the bound for each of these four values. When the signs $\pm$ are
the same, then $\tilde q = 0$ and $\bar q = \pm a$. In this case $\psi_{{\qq,\lambda,\gamma,n}}=-2(u_1\pm a)^{-1}$
does not depend on $u_2$ and ranges over a fixed bounded set for $u_1\in\supp(1-\chi)$. So in this case the first
term inside the square brackets is already bounded. 

On the other hand, if the signs $\pm$ are opposite, then $\bar q=0$ and $\tilde q = \pm a$ so 
$\psi_{{\qq,\lambda,\gamma,n}}=-2(u_1-a^2u_2^{-1})^{-1}$. In this case, even if $u_1$ remains
in the bounded set $\supp(1-\chi)$, the values of $\psi_{{\qq,\lambda,\gamma,n}}$
can approach $0\in\PA_\infty\HH$ when $u_2$ is small. So we first consider $|u_2|\ge a^2\epsilon$
for a constant $\epsilon$, to be chosen depending on $\chi$. In this case $u_1-a^2u_2^{-1}$
ranges inside a fixed bounded set for $u_1\in\supp(1-\chi)$, so again the first
term inside the square brackets is bounded. 

This leaves the case where the signs $\pm$ are opposite, $u_1\in\supp(1-\chi)$ and $|a^{-2}u_2|< \epsilon$.
In this case we find that $\psi_{{\qq,\lambda,\gamma,n}} = 2a^{-2}u_2(1-u_1a^{-2}u_2)^{-1} = a^{-2}u_2(2+O(\epsilon))
=O(\epsilon)$ so the first term in the square brackets is 
$$
\cd_{1,n}(\psi_{{\qq,\lambda,\gamma,n}}(u_1,u_2)) = {{|u_{\lambda_n-\gamma}+O(\epsilon)|^2 a^2}\over{(2+O(\epsilon))\Im(u_2)}}.
$$
The second term, with the negative sign, is 
$$
C_1 \cd_{2,n}(u_2) = C_1{{|u_{\lambda_n}+O(a^2\epsilon)|^2}\over{\Im(u_2)}}.
$$
This term dominates for $\epsilon$ sufficiently small (depending on $\chi$) and $C_1$
sufficiently large, so the quantity inside the square brackets is negative in this region.

Having justified the insertion of the cutoff function, we may write
$$\displaylines{\quad
M_{a,\alpha,\lambda,\gamma,n} 
\hfill\cr\hfill
\eqalign{
&\le \int_{\HH\times\HH} \int_{\RR^2} 2^\alpha \Big[\cd_{1,n}(\psi_{{\qq,\lambda,\gamma,n}}(u_1,u_2)) - C_1 \cd_{2,n}(u_2)\Big]_+^{1+\alpha} \chi(u_1) d\nu_a(\qq) d\rho_{a,\lambda,\gamma,n+1}(u_1,u_2)\cr
&\quad\quad + 2^\alpha C_1^{1+\alpha} M^{(2)}_{a,\alpha,\lambda,\gamma,n} + C.\cr
}
\quad}$$


Now we define
\be{twovarmudef}
\mu^0_{\qq,\lambda,\gamma,n}(u_1,u_2) = {{\cd_{1,n}(\psi_{{\qq,\lambda,\gamma,n}}(u_1,u_2)) - C_1 \cd_{2,n}(u_2)}\over{
\cd_{1,n+1}(u_1)}},
\ee
the upper bound $\mu_{\qq,\lambda,\gamma,n}(u_1,u_2)$ obtained by setting a positive term in the denominator to zero as before (the explicit formula is in the next section),
and the averaged version
$$
\overline\mu_{a,\alpha,\lambda,\gamma,n}(u_1,u_2) = \int_{\RR^2}\left[\mu_{\qq,\lambda,\gamma,n}\right]_+^{1+\alpha}(u_1,u_2) \,d\nu_a(\qq).
$$
Then, provided $|\lambda| \le \lambda_0$ so that $M^{(2)}_{a,\alpha,\lambda,\gamma,n}$ is bounded, we can rewrite the estimate above as
$$
M_{a,\alpha,\lambda,\gamma,n} \le \int_{\HH\times\HH} 2^\alpha \overline\mu_{a,\alpha,\lambda,\gamma,n}(u_1,u_2) \,\chi(u_1)  \,\cd_{1,n+1}(u_1)^{1+\alpha} d\rho_{a,\lambda,\gamma,n+1}(u_1,u_2) + C.
$$
We now perform a second iteration, followed by a second insertion of a cutoff function. 
To justify the fact that the second insertion of the cutoff function results in a bounded error $C$, we
follow the same argument as before, except that we must bound the additional
factor $\overline\mu_{a,\alpha,\lambda,\gamma,n}(\cdots)\chi(\cdots)$ (appearing on the first line of \rf{seconditer}).
%$\overline\mu_{a,\alpha,\lambda,\gamma,n}(\psi_{{\qq,\lambda,\gamma,n+1}}(u_1,u_2),\phi_{\qq,\lambda,n+1}(u_2)) %\chi(\psi_{{\qq,\lambda,\gamma,n+1}}(u_1,u_2))$. 
The fact that this quantity is bounded follows from \thmrf{finalbdd} (i)
below. We therefore
end up with the inequality
$$\displaylines{\quad
M_{a,\alpha,\lambda,\gamma,n} \le \int_{\HH\times\HH} \int_{\RR^2} 2^{2\alpha}
\overline\mu_{a,\alpha,\lambda,\gamma,n}(\psi_{{\qq,\lambda,\gamma,n+1}}(u_1,u_2),\phi_{\qq,\lambda,n+1}(u_2)) \chi(\psi_{{\qq,\lambda,\gamma,n+1}}(u_1,u_2)) 
\hfill\cr\hfill\lastdisplayline{seconditer}{
\cdot \left[\mu_{\qq,\lambda,\gamma,n+1}(u_1,u_2)\right]_+^{1+\alpha}\chi(u_1) \,d\nu_a(\qq) \,\cd_{1,n+2}^{1+\alpha}(u_1) d\rho_{a,\lambda,\gamma,n+2}(u_1,u_2) + C.\cr
\quad}}$$

\beginlemmalabel{finalbdd}
There exist $0 < \lambda_0,\lambda_1 < 2\sqrt{2}$ such that for $|\lambda|\le\lambda_0$, $|\lambda-\gamma|\le\lambda_1$,
$a$, $\alpha$ sufficiently small, $n$ sufficiently large and $\chi$ supported sufficiently near $\PA_\infty\HH$, 
\par\noindent (i) 
$$
\overline\mu_{a,\alpha,\lambda,\gamma,n}(u_1,u_2)\chi(u_1) \le C,
$$
(ii) and
there is $\epsilon>0$ such that
$$\displaylines{\quad
\int_{\RR^2} 2^{2\alpha}
\overline\mu_{a,\alpha,\lambda,\gamma,n}(\psi_{{\qq,\lambda,\gamma,n+1}}(u_1,u_2),\phi_{\qq,\lambda,n+1}(u_2)) \chi(\psi_{{\qq,\lambda,\gamma,n+1}}(u_1,u_2)) 
\hfill\cr\hfill
\cdot \left[\mu_{\qq,\lambda,\gamma,n+1}(u_1,u_2)\right]_+^{1+\alpha}\chi(u_1)d\nu_a(\qq) \le 1-\epsilon.
\quad}$$
\endlemmalabel

This lemma, proved below, implies the main result for the mean-field model.
\beginproofof{\thmrf{meanfield}} 
Inserting the estimate of \thmrf{finalbdd} (ii) into \rf{seconditer} gives
$$
M_{a,\alpha,\lambda,\gamma,n} \le (1-\epsilon)M_{a,\alpha,\lambda,\gamma,n+2} + C
$$
for $n$ large. This is the same estimate as \rf{ndep} so we can follow the argument given there
to bound $M_{a,\alpha,\lambda,\gamma,n}$ for $n$ large. As noted above, this is sufficient to  
prove the theorem.
\endproof


==> mfbdd.tex <==
\hd{8. Proof of \thmrf{finalbdd}}

The function $\mu_{\qq,\lambda,\gamma,n}(u_1,u_2)$ is the rational function given
by
$$
\mu_{\qq,\lambda,\gamma,n}(u_1,u_2)
={{|(u_2-\bar q)u_{\lambda_n-\gamma} - (u_1-\bar q)(u_2-\bar q) + \tilde q^2|^2\Im(u_1)}\over
{\big(|u_2-\bar q|^2\Im(u_1) + \tilde q^2 \Im(u_2)\big)|u_1-u_{\lambda_{n+1}-\gamma}|^2}}
-
C_1 {{\Im(u_1)|u_2-u_{\lambda_n}|_+^2}\over{\Im(u_2) |u_1-u_{\lambda_{n+1}-\gamma}|^2}}.
$$
For $|\lambda-\gamma|\le\lambda_1<2\sqrt{2}$, the fixed point $u_{\lambda_n-\gamma}$ lies in the upper half plane
for $n$ sufficiently large, and is bounded away from $\PA_\infty \HH$. The function $\mu_{\qq,\lambda,\gamma,n}(u_1,u_2)$
always appears with a cutoff function $\chi(u_1)$ that ensures that $u_1$ is in a neigbourhood of $\PA_\infty\HH$ and thus that, for $n$ sufficiently large, $|u_1-u_{\lambda_{n+1}-\gamma}|$ is bounded below
by a positive constant. The variable $u_2$ can range over all of $\HH$.
\mcomment{I don't think we ever need $u_2$ on $\PA_\infty\HH$. Its possible to make this extension, but it
involves points where $\mu$ is $-\infty$ (eg $u-2=\bar q$, $\omega_2=0$.}

Introduce polar co-ordinates $r$, $\omega_1$ and $\omega_2$ for $\Im(u_1)$ and $\Im(u_2)$ as
$$
\Im(u_1) = r\omega_1, \quad \Im(u_2) = r\omega_2, \quad \omega_1^2+\omega_2^2 = 1.
$$
Then
$$
\mu_{\qq,\lambda,\gamma,n}(u_1,u_2)={{|(u_2-\bar q)u_{\lambda_n-\gamma} - (u_1-\bar q)(u_2-\bar q) + \tilde q^2|^2\omega_1}\over
{\big(|u_2-\bar q|^2\omega_1 + \tilde q^2 \omega_2\big)|u_1-u_{\lambda_{n+1}-\gamma}|^2}}
-
C_1 {{\omega_1|u_2-u_{\lambda_n}|_+^2}\over{\omega_2 |u_1-u_{\lambda_{n+1}-\gamma}|^2}}.
$$
With a Bernoulli distribution, the potential takes on four possible values $(\pm a,\pm a)$.
The corresponding values of $\mu$ are as follows.
$$
\mu^{++}_{a,\lambda,\gamma,n}(u_1,u_2) = 
{{|u_1- u_{\lambda_n-\gamma} -a|^2}\over
{|u_1-u_{\lambda_{n+1}-\gamma}|^2}}
-
C_1 {{\omega_1|u_2-u_{\lambda_n}|_+^2}\over{\omega_2 |u_1-u_{\lambda_{n+1}-\gamma}|^2}}.
$$
The formula for $\mu^{--}$ is identical, except that $-a$ is replaced with $a$. For the other two
values, we have $\mu^{+-} = \mu^{-+}$, with
$$
\mu^{+-}_{a,\lambda,\gamma,n}(u_1,u_2) = 
{{|u_2(u_1 - u_{\lambda_n-\gamma}) - a^2|^2\omega_1}\over
{\big(|u_2|^2\omega_1 +a^2 \omega_2\big)|u_1-u_{\lambda_{n+1}-\gamma}|^2}}
-
C_1 {{\omega_1|u_2-u_{\lambda_n}|_+^2}\over{\omega_2 |u_1-u_{\lambda_{n+1}-\gamma}|^2}}.
$$
\beginlemma For $u_1$ in a neigbourhood of $\PA_\infty\HH$ and $a$ bounded,
$$
\mu^{++}_{a,\lambda,\gamma,n}(u_1,u_2) \le 1 + C{{a + 2^{-n}}\over{|u_1-u_{\lambda_{n+1}-\gamma}|}}.
$$
\endlemma
\beginproof
Dropping the second term we have
$$
\mu^{++}_{a,\lambda,\gamma,n}(u_1,u_2) \le \left|1 + {{u_{\lambda_{n+1}-\gamma}-u_{\lambda_n-\gamma}-a}\over{u_1-u_{\lambda_{n+1}-\gamma}}}\right|^2.
$$
Expanding the square, using that
$|u_{\lambda_n-\gamma}-u_{\lambda_{n+1}-\gamma}|\le C2^{-n}$
and that
$|(a + C2^{-n})/(u_1-u_{\lambda_{n+1}-\gamma})|$ is bounded, since $a$ is bounded
and $u_1$ is bounded away from $u_{\lambda_{n+1}-\gamma}$ near $\PA_\infty\HH$ completes the proof.
\endproof
The following lemma is the most involved estimate in this section.
\beginlemma Suppose that $u_1$ lies in a sufficiently small neighbourhood of infinity. Then for
$C_1$ and $n$ suffciently large and $a$ sufficiently small, there exists a positive constant $C$ such that
\be{pmbdd}
\mu^{+-}_{a,\lambda,\gamma,n}(u_1,u_2) \le 1 - {{C\sqrt{C_1}(a-2^{-n})}\over{|u_1-u_{\lambda_{n+1}-\gamma}|}}.
\ee
\endlemma
\beginproof
To simplify the appearance of the formulas, we introduce the notation
$$
A_n = u_1 - u_{\lambda_n-\gamma}, \quad B_n = u_2-u_{\lambda_n}.
$$
We begin by establishing the inequality
\be{firstmubdd}
\mu^{+-}_{a,\lambda,\gamma,n}(u_1,u_2) \le {{\left[ |u_2A_n-a^2| - a\sqrt{C_1}|B_n|_+\right]_+^2}\over{|u_2|^2|A_{n+1}|^2}}.
\ee
Let $x=\omega_2/\omega_1 \in [0,\infty]$. We must maximize
$$
\mu^{+-}_{a,\lambda,\gamma,n}(u_1,u_2) = {{|u_2A_n-a^2|^2}\over{(|u_2|^2 + xa^2)|A_{n+1}|^2}}
- C_1{{|B_n|_+^2}\over{x|A_{n+1}|^2}}
$$
over $x$. We will assume without loss that $a>0$. Differentiating with respect to $x$ we obtain the 
following equation for the critical point:
$$
{{|u_2A_n-a^2|^2a^2}\over{(|u_2|^2 + xa^2)^2}} = {{C_1 |B_n|_+^2}\over{x^2}},
$$
or
$$
|u_2A_n-a^2|ax = \pm \sqrt{C_1}|B_n|_+(|u_2|^2 + xa^2).
$$
Since $x$ is non-negative we must choose $\pm = +$. This results in the critical point
$$
x = {{\sqrt{C_1}|B_n|_+|u_2|^2}\over{a (|u_2A_n-a^2| - a \sqrt{C_1}|B_n|_+)}}.
$$
The critical point will lie in $[0,\infty]$ provided
\be{critineq}
|u_2A_n-a^2| \ge a \sqrt{C_1}|B_n|_+,
\ee
in which case a calculation shows that the critical value is
\be{critval}
{{\left(|u_2A_n-a^2| - a\sqrt{C_1}|B_n|_+\right)^2}\over{|u_2|^2|A_{n+1}|^2}}.
\ee
At the endpoint $x=0$ we find that $\mu^{+-}$ tends to $-\infty$ while the limit as $x\rarr\infty$ is $0$.
This implies that when \rf{critineq} holds, then the maximum occurs at the critical value, and otherwise the maximum
is $0$. This proves \rf{firstmubdd}.

Now we can proceed with the proof of estimate \rf{pmbdd}. We may assume that \rf{critineq} holds, because
otherwise $\mu^{+-}$ is zero and the desired estimate is true. This implies that for some $\epsilon >0$
$$
|u_2A_n| \ge a(1-\epsilon)\sqrt{C_1}|B_n|_+
$$
for $a$ small and $C_1$ large enough. Here we use that $|B_n|_+ \ge C$. Thus we may assume
\be{mayassume}
{{a\sqrt{C_1}|B_n|_+}\over{|u_2A_n|}}\le 1+2\epsilon
\ee
provided $0<\epsilon<1/2$ and use this in estimating \rf{critval}. Expanding the square in \rf{critval}
we end up with an estimate for $\mu^{+-}$ given by
$$\displaylines{
\mu^{+-}_{a,\lambda,\gamma,n}(u_1,u_2) \le
{{|A_n|^2}\over{|A_{n+1}|^2}}
\hfill\cr\hfill 
+ 
{{a|B_n|_+}\over{|u_2||A_{n+1}|}}\left(
{{2a|A_n|}\over{|A_{n+1}||B_n|_+}} + 
{{a^3}\over{|u_2||A_{n+1}||B_n|_+}} - {{2\sqrt{C_1}|A_n|}\over{|A_{n+1}|}} 
+ {{2\sqrt{C_1}a^2}\over{|u_2||A_{n+1}|}} 
+ {{C_1a|B_n|_+}\over{|u_2||A_{n+1}|}}\right).
\cr}$$
Now we may use \rf{mayassume}, $|B_n|_+ \ge C$ and $|A_n|/|A_{n+1}| \le 1 + C2^{-n}/|A_{n+1}|$ to arrive at
the estimate
$$
\mu^{+-}_{a,\lambda,\gamma,n}(u_1,u_2)\le 1 + C2^{-n}/|A_{n+1}| - {{a|B_n|_+}\over{|u_2||A_{n+1}|}}((1-2\epsilon)\sqrt{C_1} - Ca).
$$
Finally, the bound $|B_n|_+/|u_2| \ge C$ completes the proof.
\endproof

\beginproofof{\thmrf{finalbdd}}
With the Bernoulli distribution, the average defining $\overline\mu$ has four terms, so,
dropping the subscripts and using the estimates from this section we have
$$\eqalign{
\overline\mu(u_1,u_2) 
&= {{1}\over{4}} \left(
[\mu^{++}]_+^{1+\alpha} + [\mu^{--}]_+^{1+\alpha} +[\mu^{+-}]_+^{1+\alpha} +[\mu^{-+}]_+^{1+\alpha} 
\right)\cr
&\le {{1}\over{2}} \left(
\left[1 + C{{a+2^{-n}}\over{|u_1-u_{\lambda_{n-1}-\gamma}|}}\right]^{1+\alpha}
+\left[1 - C\sqrt{C_1}{{a-2^{-n}}\over{|u_1-u_{\lambda_{n-1}-\gamma}|}}\right]^{1+\alpha}
\right).
}$$
Part (i) of the lemma follows immediately from this estimate. 

Continuing with the proof of (ii),
for $a$ small and $n$ large, both terms inside the square brackets are a small perturbation of $1$.  But
since we are free to take $C_1$ large, we may assume that the relative size of the term with the good (negative)
sign is much larger. This leads to the estimate 
$$
\overline\mu(u_1,u_2) \le 1 - C\sqrt{C_1}{{a-2^{-n}}\over{|u_1-u_{\lambda_{n-1}-\gamma}|}} 
+ C (a+2^{-n})^2
$$
for $a$, $\alpha$ small and $n$, $C_1$ large.

To prove the lemma we must estimate the expression (again dropping most subscripts)
$$
{{1}\over{4}} \sum_{\qq \in (\pm a,\pm a)}
2^{2\alpha}
\overline\mu(\psi_\qq(u_1,u_2),\phi_\qq(u_1,u_2))\,\chi(\psi_\qq(u_1,u_2))\;
[\mu_\qq(u_1,u_2)]_+^{1+\alpha}\,\chi(u_1)
$$
When $|u_1|\le C$ we can estimate $\overline\mu$ by $1+ C (a+2^{-n})^2$ and pull it out of the sum.
What results is another copy of $\overline\mu$ evaluated at bounded $u_1$. This can be estimated
by $1-\epsilon$. Since for small $\alpha$ the quantity $2^{2\alpha}$ is close to $1$, we end up
with the desired bound of $1-\epsilon$ for $a$, $\alpha$ small and $n$, $C_1$ large.

For $u_1$ near infinity we estimate the occurances of $\mu$ in the sum by the bound for $\mu^{++}$ which is slightly
greater than one. Then we just need to guarantee that one of the $\overline\mu$ terms will be evaluated
with $\psi_\qq(u_1,u_2)$ bounded. This happens when $\qq = (a,a)$ since in this case 
$\psi_\qq(u_1,u_2) = -2/(u_1-\bar q)+\lambda_n-\gamma$ independently of $u_2$.
\endproof


==> mubdd.tex <==
\hd{6. Proof of \thmrf{mubarbdd}}

The goal of this section is to prove the estimates in \thmrf{mubarbdd} on $\mu$ defined by \rf{mudef} for $u$ and $\lambda$ real.
Notice that when $\lambda\in\RR$ and $|\lambda| < 2\sqrt{2}$ then $\Im(u_\lambda) > 0$ and $|u_\lambda|^2 = 2$.

We will blow up the singularity on the diagonal by introducing polar co-ordinates $r$ and $\omega_i$, $i=1,2$ defined by
$$
u-q_1 = r\omega_1, \quad u-q_2 = r\omega_2, \quad \omega_1^2 + \omega_2^2 = 1.
$$

We begin with the estimate for $|u|$ small.
\beginlemmalabel{mubdd1}
Suppose $|\lambda| < 2\sqrt{2}$, $|q_i|\le a$ and $|u|\le aR$ where $R\ge 2$ and $aR\le 1/4$. Then
$$
\mu_{\qq,\lambda}(u) \le {{|\omega_1+\omega_2|^2}\over{2}} + CaR.
$$
\mcomment{In fact $C \sim 12.59$.}
\endlemma
\beginproof
We can write
$$
\mu_{\qq,\lambda}(u) = {{|(\omega_1+\omega_2)u_\lambda + 2r\omega_1\omega_2|^2}\over{2|u-u_\lambda|^2}}.
$$
We have
$$
{{2}\over{|u-u_\lambda|^2}} = {{2}\over{2-\lambda u + u^2}} \le {{1}\over{1-\lambda u/2}} \le 1 + |\lambda||u|
$$
since $|\lambda u/2|\le 1/2$ and $(1-x)^{-1} \le 1 + 2 |x|$ for $|x|\le 1/2$. Next, we have
$$
{{|(\omega_1+\omega_2)u_\lambda + 2r\omega_1\omega_2|^2}\over{4}} \le {{|\omega_1 + \omega_2|^2}\over{2}} + r + r^2/4,
$$
since $|\omega_1 + \omega_2|<\sqrt{2}$, $|\omega_1\omega_2|\le1/2$. With our bounds on $q_i$ and $R$ we have
$$
r^2 = |u-q_1|^2 + |u-q_2|^2 \le 2a^2(1+R)^2.
$$
Combining these estimates completes the proof.
\endproof

Now we turn to the estimate for large $|u|$.
\beginlemmalabel{mubdd2}
Suppose $|\lambda| < 2\sqrt{2}$, $|q_i|\le a$ and $|u|\ge aR$ where $R\ge 2$. Then
$$
\mu_{\qq,\lambda}(u) \le 1 + {{1}\over{u}}\jap{{\bf l}, \qq}
- {{1}\over{u^2}}\jap{\qq,(Q-C/R)\qq}
$$
with
$$\eqalign{
\qq&=\twomat{q_1}{q_2},\cr
{\bf l} &= {{-2u^2+\lambda u}\over{2|u-u_\lambda|^2}}\twomat{1}{1},\cr
Q &= {{1}\over{2|u-u_\lambda|^2}}\twomat{u^2-\lambda u + 1 & -2u^2+\lambda u - 1}{-2u^2+\lambda u - 1 & u^2-\lambda u + 1}.
}$$
The constant $C = C_1/(1-\lambda^2/8) + C_2$ where $C_1$ and $C_2$ are numbers.
\endlemmalabel
\beginproof
Let $\delta_i = q_i/u$ and note that $|\delta_i|< 1/R$. We can write 
\be{muproduct}
\mu_{\qq,\lambda}(u)={{1}\over{4|u-u_\lambda|^2}}
|2(u-u_\lambda) - (\delta_1+\delta_2)(2u-u_\lambda)+2\delta_1\delta_2u|^2
{{2}\over{|1-\delta_1|^2 + |1-\delta_2|^2}}.
\ee
The third term on the right can be written
$$
{{2}\over{|1-\delta_1|^2 + |1-\delta_2|^2}} = {{1}\over{1-(\delta_1+\delta_2) + (\delta_1^2+\delta_2^2)/2}}.
$$
If $x\le\delta<1$ then $(1-x)^{-1} \le 1+x+(1+\delta/(1-\delta))x^2$. Using this with $x=(\delta_1+\delta_2) - (\delta_1^2+\delta_2^2)/2$ and $\delta = (2R-1)/R^2$, which implies $\delta/(1-\delta)\le 6/R$ we find, after some calculation, that this term can be estimated by
$$
{{2}\over{|1-\delta_1|^2 + |1-\delta_2|^2}}\le 1+(\delta_1+\delta_2) + 2\delta_1\delta_2 + \left({{1}\over{2}}+{{40}\over{R}}\right)(\delta_1^2+\delta_2^2).
$$
We now turn to the middle term on the right side of \rf{muproduct}. Multiplying out the square, using $\Re(u_\lambda)=\lambda/2$, and making some simple estimates, we arrive at
$$\displaylines{\quad\quad
|2(u-u_\lambda) - (\delta_1+\delta_2)(2u-u_\lambda)+2\delta_1\delta_2u|^2
\hfill\cr\hfill
\eqalign{
&\le 4|u-u_\lambda|^2 - 4(\delta_1+\delta_2)(|u-u_\lambda|^2 + u(u-\lambda/2)) \cr
&\quad + 2\delta_1\delta_2(|2u-u_\lambda|^2+4u(u-\lambda/2))\cr
&\quad + (\delta_1^2+\delta_2^2)(|2u-u_\lambda|^2 + R^{-1}(9|u|^2 +2|\lambda u|)).\cr
}\quad\quad}$$
We now combine these estimates. In the error terms, we can control quadratic terms in $u$ using
$$
|u|^2 \le {{1}\over{1-\lambda^2/8}}|u-u_\lambda|^2.
$$
A straightforward calculation completes the proof.
\endproof

In preparation for the proof of \thmrf{mubarbdd} we prove the following lemma. Recall that $\omega_1$ and $\omega_2$ are functions of $u$ and $\qq$. Explicitly,
$$
\omega_i(u,\qq) = {{u-q_i}\over{\sqrt{(u-q_1)^2+(u-q_2)^2}}},
$$
so that $\omega_i(u,a\qq) = \omega_i(u/a,\qq)$.
Also, with the notation of \rf{nuassn2} we have
$$
\int_{\RR^2} (q_1-q_2)^2 d\nu(\qq) = c_{11}+c_{22}-2c_{12} = c(1-\delta).
$$

\beginlemmalabel{omegaint}
For $R\ge 2$ and $|u|\le a R$,
\be{omegaintbdd}
\int_{\RR^2}{{|\omega_1+\omega_2|^2}\over{2}} d\nu_a(\qq) \le 1 - {{c(1-\delta)}\over{20 R^2}}.
\ee
\endlemmalabel
\beginproof
We begin with a scaling argument. The scaling properties of $\omega_i(u,\qq)$ and $\nu_a$ imply
that bounding the left side of \rf{omegaintbdd} for $|u|\le aR$ is equivalent to
bounding
$$
\int_{\RR^2}{{|\omega_1+\omega_2|^2}\over{2}} d\nu(\qq)
$$
for $|u|\le R$.

Referring to the following diagram, we have $\omega_1=-\cos(\theta + \pi/4)$ and $\omega_2=-\sin(\theta + \pi/4)$.
\vskip 20pt
\epsfxsize=4cm
\centerline{\epsffile{omega.eps}}

Then $|\omega_1+\omega_2|^2/2 = (1 + 2\omega_1\omega_2)/2 = (1+\cos(2\theta))/2$. From this we see that the maximum 
occurs at an endpoint for $\theta$, when $(u,u) = (R,R)$ or $(u,u) = (-R,-R)$. This leads to
$$
{{|\omega_1+\omega_2|^2}\over{2}} 
\le{{|\pm R - \bar q|^2}\over{|\pm R - \bar q|^2 + \tilde q^2}}
=1-{{\tilde q^2}\over{|R\pm \bar q|^2 + \tilde q^2}},
$$
where $\bar q = (q_1+q_2)/2$ and $\tilde q = (q_1-q_2)/2$. Since $|\bar q|\le 1$ and $R\ge 2$ we have $|R\pm \bar q|\le 2R$.
This implies
$$
{{|\omega_1+\omega_2|^2}\over{2}} \le 1-{{\tilde q^2}\over{4R^2+1}} = 1-{{(q_1-q_2)^2}\over{20R^2}}.
$$
Integrating this formula completes the proof.
\endproof

We are now ready to give the proof of \thmrf{mubarbdd}.

\beginproofof{\thmrf{mubarbdd}}
The estimates of \thmrf{mubdd1}, \thmrf{mubdd2} and the estimate
$(1+x)^{1+\alpha} \le 1 + (1+\alpha)x + \alpha(1+\alpha)x^2$ for $x>-1$ can be used to show
$$
\mu_{\qq,\lambda}(u)^{1+\alpha} \le
\cases{\displaystyle{
{{|\omega_1+\omega_2|^2}\over{2}} + C_1aR + C_2\alpha}
& for $|u| \le aR$
\cr
\displaystyle{
1 + {{1+\alpha}\over{u}}\jap{{\bf l}, \qq}
- {{1}\over{u^2}}\jap{\qq,(Q-C_3/R-C_4\alpha)\qq}}
& for $|u| \ge aR$
\boxhwt{25pt}{0pt}{0pt}\cr
}.
$$
We now integrate this estimate with respect to $\nu_a$. For $|u| \le aR$, we use \thmrf{omegaint}.
When we integrate the estimate for  $|u| \ge aR$, the linear term vanishes, thanks to \rf{nuassn3}.
The quadratic term gives the estimate on the right side in \rf{mubarbdd}.
\endproof


==> refs.tex <==
\vfill\eject
\hd{Acknowledgements}
We would like to thank the University of Erlangen-N\"urnberg (R.F.),
the University of British Columbia and the Erwin Schr\"odinger Institut
(D.H. and W.S.), and Jacobs University (W.S.) for hospitality and
financial support.

\hd{References}
\parindent = 0pt
\tolerance = 1000

[AF] C.~Allard and  R.~Froese, {\it A Mourre estimate for a Schr\"odinger operator
on a binary tree}, Rev.\ Math.\ Phys.\  12,  no.~12, 1655--1667, 2000, {\tt mp-arc:98-497}.

[ASW] M.~Aizenman, R.~Sims and S.~Warzel, {\it Stability of the Absolutely 
Continuous Spectrum of Random Schr\"odinger Operators on Tree Graphs,}
Prob.~Theor.~Rel.~Fields, {\bf 136}, No.~3, 363--394, 2006, {\tt arXiv:math-phys/0502006}.

[B1] J.~Breuer, {\it  Localization for the Anderson Model on Trees with Finite Dimensions},
Annales Henri Poincar\'e, {\bf 8}, No.~8, 1507--1520, 2007, {\tt arXiv:math/0609474}.

[B2] J.~Breuer, {\it Singular continuous spectrum for the Laplacian on certain
sparse trees},  Comm.\ Math.~Phys., {\bf 269}, No.~3, 851-857, 2006, {\tt arXiv:math/0608159}.

[BF] J.~Breuer and R.~L.~Frank, {\it Singular spectrum for radial trees}, {\tt arXiv:0806.0649}.

[FHS1] R.~Froese, D.~Hasler and W.~Spitzer, {\it Transfer matrices, hyperbolic
geometry and absolutely continuous spectrum for some discrete Schr\"odinger 
operators on graphs}, J.~Func.~Anal., {\bf 230}, No.~1, 184--221, 2005, {\tt mp-arc:04-244}.

[FHS2] R.~Froese, D.~Hasler and W.~Spitzer, {\it Absolutely Continuous Spectrum for the Anderson Model on a Tree: A Geometric Proof of Klein's Theorem}, Comm.~Math.~Phys., {\bf 269}, No.~1, 239--257, 2007, {\tt mp-arc:05-388}.

[H] F.~Halasan, U.B.C.\ Thesis in preparation.

[K] A.~Klein, {\it Extended States in the Anderson Model on the Bethe
Lattice}, Advances in Math., {\bf 133}, 163--184, 1998, {\tt mp-arc:94-236}.
                                 
[Si] B.~Simon, {\it $L^p$ Norms of the Borel Transform and the Decomposition of Measures}, Proc.~A.M.S., {\bf 123}, No.~12, 3749--3755, 1995.

[Sp] W.~Spitzer, {\it Absolutely Continuous Spectrum on some Tree
Graphs}, Oberwolfach Report No. 12/2007, Transport in multi-dimensional
random-Schr\"odinger operators.


==> rixmax.tex <==
\input amssym.def
%\def\Bbb{\bf} %if \Bbb not available
 
%fonts

\font\bold=cmssbx10
\font\smallfont = pplr at 8.5pt
\font\smallit = pplri at 8.5pt
\font\normalfont = pplr at 9.5pt
\font\it = pplri at 9.5pt
\font\marginfont=cmr7

\def\pplfonts{
	\font\tenrm=pplr at 9.5pt
	\font\tensl=pplro at 9.5pt
	\font\eightit=pplri at 8.5 pt
	\tenrm
}


% shorthand
 
\def\larr{\leftarrow}
\def\rarr{\rightarrow}
\def\uarr{\uparrow}
\def\darr{\downarrow}
\def\PA{\partial}
\def\ti{\tilde}
\def\<{\langle}
\def\>{\rangle}
\def\cents{\hbox{\rm\rlap/c}}

% single letters

\def\HI{{\cal H}}
\def\HH{{\Bbb H}}
\def\RR{{\Bbb R}}
\def\CC{{\Bbb C}}
\def\ZZ{{\Bbb Z}}
\def\NN{{\Bbb N}}
\def\MM{{\cal M}}
\def\QQ{{\Bbb Q}}
\def\DD{{\cal D}}
\def\FF{{\cal F}}
\def\BB{{\cal B}}
\def\GG{{\cal G}}
\def\SS{{\bf S}}
\def\TT{{\bf T}}
\def\EE{{\cal E}}
\def\UU{{\cal U}}
\def\II{{\cal I}}
\def\OO{{\cal O}}
\def\Fb{{\bf F}}
\def\ib{{\bf i}}
\def\jb{{\bf j}}
\def\kb{{\bf k}}
\def\rb{{\bf r}}
\def\vb{{\bf v}}
\def\hb{{\bf h}}
% misc math stuff

\def\slim{\mathop{\hbox{\rm s-lim}}}
\def\Ker{\mathop{\rm Ker}}
\def\Ran{\mathop{\rm Ran}}
\def\ad{\mathop{\rm ad}}
\def\Re{\mathop{\rm Re}}
\def\Im{\mathop{\rm Im}}
\def\Log{\mathop{\rm Log}}
\def\Arg{\mathop{\rm Arg}}
\def\tr{\mathop{\rm tr}}
\def\curl{\mathop{\bold curl}}
\def\div{\mathop{\bold div}}
\def\ess{\hbox{\it ess}}
\def\d{\hbox{\it d}}
\def\c{\hbox{\it c}}
\def\pp{\hbox{\it pp}}
\def\jap#1{\langle #1 \rangle}
\def\sph{S^{n\kern -.2ex -\kern -.2ex 1}}
\def\half{$\scriptstyle{{1}\over{2}}$}
\def\DT{{{\partial}\over{\partial t}}}
\def\L{\Delta}
\def\norm#1{\|#1\|}
\def\dint{\int\hskip -5pt \int}
\def\trint{\int\hskip -5pt \int\hskip -5pt \int}
\def\amat4#1#2#3#4#5#6#7#8{
\left[\matrix{
#1\cr
#3\cr
#5\cr
#7\cr
}\right.\left|\matrix{
#2\cr#4\cr#6\cr#8\cr
}\right]
}

\def\vec4#1#2#3#4{
\left[\matrix{
#1\cr
#2\cr
#3\cr
#4\cr
}\right]
}

\def\amat3#1#2#3#4#5#6{
\left[\matrix{
#1\cr
#3\cr
#5\cr
}\right.\left|\matrix{
#2\cr#4\cr#6\cr
}\right]
}

\def\vec3#1#2#3{
\left[\matrix{
#1\cr
#2\cr
#3\cr
}\right]
}
 
\def\amat2#1#2#3#4{
\left[\matrix{
#1\cr
#3\cr
}\right.\left|\matrix{
#2\cr#4\cr
}\right]
}
\def\vec2#1#2{
\left[\matrix{
#1\cr
#2\cr
}\right]
}
 
\def\threevec#1#2#3{
\left[\matrix{
#1\cr
#2\cr
#3\cr
}\right]
}

\def\twovec#1#2{
\left[\matrix{
#1\cr
#2\cr
}\right]
}

\def\tr{{\rm tr}}
\def\div{\hbox{\bold div}}
\def\curl{\hbox{\bold curl}}
% misc


%
% 	the stuff after \ifdraftmode only appears if \draftmode has previously 
%	appeared
%
\def\draftmode{\let\dfmd 1}
\def\ifdraftmode#1{\ifx\dfmd 1{#1}\fi}

\def\today{\ifcase\month\or January\or February \or March \or April\or May\or June\or July\or August\or September\or October \or November \or December\fi
\space\number\day, \number\year}

\def\nnarrower{\advance\leftskip by 30pt\advance\rightskip by 30pt}

\def\wwider{\advance\leftskip by -30pt\advance\rightskip by -30pt}

\def\quote#1{{\smallskip\nnarrower\noindent{\it#1}\smallskip}}

\def\hd#1{
\par\penalty-5000
\bigskip\bigskip{\noindent\bold #1}\par\vrule height\bigskipamount width 0pt\penalty10000
}

\def\enum#1{\par\noindent\quad\rlap{#1}\hskip 20pt}

\def\Box{\vbox{\hrule
              \hbox{\vrule height7pt\kern7pt\vrule height7pt}
              \hrule
              }
        }

\def\Picbox{\centerline{
		\vbox{\hrule
                \hbox{\vrule height2.5in\kern5in\vrule height2.5in}
                \hrule
                }
	    }
        }

% 
%	a box of specified height, width and thickness
%

\def\boxhwt#1#2#3{\vbox{\hrule width#2 height#3
                	\hbox{\vrule height#1 width#3 \kern#2\kern-#3\kern-#3 \vrule height#1 width#3}
                	\hrule width#2 height#3
                	      }
        	}
%
%
%	mcomment puts a comment in the margins
%
%
%
%
\def\strutdepth{\dp\strutbox}
%
\newdimen\pagewidth
\newdimen\marginsize

\def\margininsert#1{\strut\vadjust{\kern-\strutdepth
\vtop to \strutdepth{\baselineskip\strutdepth\vss\llap{\marginfont #1}\null}}}
%
\def\marginbox#1{{
\pagewidth=8.5 true in
%	set \marginsize to 1in + \hoffset - .26 true in
	\marginsize=1 true in
	\advance \marginsize by \hoffset
	\advance \marginsize by -.26 true in
\parindent=0pt\raggedright\hsize = \marginsize\vbox{#1}\kern 3pt}}
%
%
\def\mcomment#1{\margininsert{\marginbox{#1}}}

%
%       the following macros read in the files \jobname.eqr 
%       and \jobname .thm which 
%       contain the names of equations and how they are nested 
%       within sections in a format like 
%       \\{name1}\bgnscn\\{name2}\bgnscn\\{name3}\ndscn\ndscn
%       In this example \eqlabelname1 will expand to 1
%                       \eqlabelname2 will expand to 1.1
%                       \eqlabelname3 will expand to 1.1.1
%       This is the maximum nesting supported
%       In the theorem list each \\{name} is preceded by \typetheorem,
%       \typelemma or \typeproposition to indicate what it is
%



\def\bgnsctn{
        \advance\secnest by1
        \cntnumber=0
        \ifnum\secnest=1 
                \advance\seclevelone by1 
                \edef\prenum{\number\seclevelone .}
        \fi
        \ifnum\secnest=2 
                \advance\secleveltwo by1
                \edef\prenum{\number\seclevelone .\number\secleveltwo .}
        \fi
        }
\def\ndsctn{\advance\secnest by-1}

\def\thmtype{} %initialize
\def\typetheorem{\def\thmtype{Theorem}}
\def\typelemma{\def\thmtype{Lemma}}
\def\typeproposition{\def\thmtype{Proposition}}
\def\typecorollary{\def\thmtype{Corollary}}
\def\typehypothesis{\def\thmtype{Hypothesis}}
\def\typeconjecture{\def\thmtype{Conjecture}}
%
% first do the references - define \\ to be a macro which defines \eqlabelname 
% to be a reference number and then evaluate the input string as in Appendix D
%
\def\\#1{
        \advance\cntnumber by1
        \expandafter\xdef\csname 
        eqlabel#1\endcsname{\prenum\number\cntnumber}
        }
\newcount\seclevelone \seclevelone=0
\newcount\secleveltwo \secleveltwo=0
\newcount\cntnumber \cntnumber=0
\newcount\secnest \secnest=0
\def\prenum{}
\newread\eqrinfile 
\openin\eqrinfile=\jobname .eqr 
\ifeof\eqrinfile
  \def\eqrinput{\relax}
\else\loop
  \read\eqrinfile to\eqrinput
  \eqrinput
  \ifeof\eqrinfile\let\endfile 1\else\let\endfile 0\fi
  \ifx\endfile 0 \repeat
\fi
\closein\eqrinfile

%
% now the same thing for theorems
%
\def\\#1{
        \advance\cntnumber by1
        \expandafter\xdef\csname 
        thmlabel#1\endcsname{\prenum\number\cntnumber}
        \expandafter\xdef\csname 
        typethmlabel#1\endcsname{\thmtype\ \prenum\number\cntnumber}
        }
\seclevelone=0
\secleveltwo=0
\cntnumber=0
\secnest=0
\def\prenum{}
\newread\thminfile 
\openin\thminfile=\jobname .thm
\ifeof\thminfile
  \def\thminput{\relax}
\else\loop
  \read\thminfile to\thminput
  \thminput
  \ifeof\thminfile\let\endfile 1\else\let\endfile 0\fi
  \ifx\endfile 0 \repeat
\fi
\closein\thminfile


        
%
% theorems etc
% These are numbered by section
%

\def\begintheoremlabel#1{
       	\toksdef\ta=0
	\ta={\typetheorem\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Theorem \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endtheoremlabel{\par\medbreak\endgroup}

\def\begintheorem{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\begintheoremlabel\temp
}
\def\endtheorem{\endtheoremlabel}

\def\beginlemmalabel#1{
        \toksdef\ta=0
	\ta={\typelemma\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Lemma \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endlemmalabel{\par\medbreak\endgroup}

\def\beginlemma{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginlemmalabel\temp
}
\def\endlemma{\endlemmalabel}



\def\beginpropositionlabel#1{
        \toksdef\ta=0
	\ta={\typeproposition\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Proposition \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endpropositionlabel{\par\medbreak\endgroup}

\def\beginproposition{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginpropositionlabel\temp
}
\def\endproposition{\endpropositionlabel}

\def\begincorollarylabel#1{
        \toksdef\ta=0
	\ta={\typecorollary\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Corollary \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endcorollarylabel{\par\medbreak\endgroup}

\def\begincorollary{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\begincorollarylabel\temp
}
\def\endcorollary{\endcorollarylabel}

\def\beginhypothesislabel#1{
        \toksdef\ta=0
	\ta={\typehypothesis\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Hypothesis \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endhypothesislabel{\par\medbreak\endgroup}

\def\beginhypothesis{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginhypothesislabel\temp
}
\def\endhypothesis{\endhypothesislabel}

\def\beginconjecturelabel#1{
       	\toksdef\ta=0
	\ta={\typeconjecture\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Conjecture \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endconjecturelabel{\par\medbreak\endgroup}

\def\beginconjecture{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginconjecturelabel\temp
}
\def\endconjecture{\endconjecturelabel}





\def\beginproof{\medbreak\par\noindent{\it Proof:\/\ }}
\def\endproof{\thinspace\Box\par\medbreak}

\def\beginproofof#1{\medbreak\par\noindent{\it Proof of #1:\/\ }}
\def\endproofof{\thinspace\Box\par\medbreak}



\def\begindefn{\medbreak\par\noindent{\it Definition:\/\ }}
\def\enddefn{\par\medbreak}

\def\beginexample{\medbreak\par\noindent{\it Example:\/\ }}
\def\endexample{\par\medbreak}

\def\beginexampleset{\beginproblemset}
\def\endexampleset{\endproblemset}


\def\beginremark{\medbreak\par\noindent{\it Remark:\/\ }}
\def\endremark{\par\medbreak}

\def\beginremarkno#1{\medbreak\par\noindent{\it Remark #1:\/\ }}
\def\endremarkno{\par\medbreak}



%-------------------------------------------------------
%	no longer needed
%
%       \appendtxt appends the text in #2 to the token list 
%       contained in the token variable #1
%
\def\appendtxt#1#2{ 
        \toksdef\ta=0
        \ta=\expandafter{\the#1#2}
        \global#1=\expandafter{\the\ta}
        }
%----------------------------------------------------------

%
%
%	open files for writing
%
%
\newwrite\eqroutfile 
\immediate\openout\eqroutfile=\jobname .eqr 
\newwrite\thmoutfile 
\immediate\openout\thmoutfile=\jobname .thm


%
%       \be{name} and \ee begin and end a numbered displayed equation 
%       the tokens in the name are added to the token list in \eqrtoks
%       if \eqlabelname has been defined uses this as a number
%       \lastdisplayline{name}{...} gives a referenced number  to the last 
%       line in a displaylines series
%
\def\be#1{
        \def\temp{#1}
	\toksdef\ta=0
	\ta={\\{#1}}
        \immediate\write\eqroutfile{\the\ta}$$
	}
\def\ee{
        \eqno{(\csname eqlabel\temp\endcsname)
	\ifdraftmode{\rlap{\ {\marginfont\temp}}}}$$
        }
\def\lastdisplayline#1#2{
        \hfill#2\hfill{\rm\llap{(\csname eqlabel#1\endcsname)}
	\ifdraftmode{\rlap{\ {\marginfont#1}}}}\cr
        \toksdef\ta=0
	\ta={\\{#1}}
        \immediate\write\eqroutfile{\the\ta}
        }

%
%       \beginsection begins a new section
%       writes \bgnsctn to token list in \eqrtoks
%       \endsection ends a section
%       writes \ndsctn to token list in \eqrtoks
%
\def\beginsection{
        \advance\secnumber by1
        \probctr=0
	\toksdef\ta=0
	\ta={\bgnsctn}
        \immediate\write\eqroutfile{\the\ta}
        \immediate\write\thmoutfile{\the\ta}
        }
\def\endsection{
        \toksdef\ta=0
	\ta={\ndsctn}
        \immediate\write\eqroutfile{\the\ta}
        \immediate\write\thmoutfile{\the\ta}
        }

%
%       \rf{name} inserts (<number>) where <number> is the equation number
%       referred to by "name"
%
\def\rf#1{(\csname eqlabel#1\endcsname )}

%
%       \thmrf is the analogous thing for theorems
%
%\def\thmrf#1{\hbox{\csname typethmlabel#1\endcsname}}
\def\thmrf#1{\csname typethmlabel#1\endcsname}







\def\chead#1{\medbreak\centerline{#1}\medskip}

\def\bea#1{$$\eqalign\begingroup}
\def\eea{\endgroup $$}
\def\beann{$$\eqalign\begingroup}
\def\eeann{\endgroup $$}


%
%       some lecture note macros
%
\def\beginlecture{
        \beginsection 
        \probctr=0
        \par\noindent{\bf Lecture \number\secnumber}
        \medskip
}
\def\endlecture{\endsection\vfill\eject}
%
%
%
\def\beginlecturetitle#1{
        \beginsection 
        \probctr=0
        \par\noindent{\bf Lecture \number\secnumber : #1}
        \medskip
}
\def\endlecturetitle{\endsection\vfill\eject}
%
%
%
\def\readsec#1{\medskip{\sl Reading:} Section #1}
\def\readsecs#1{\medskip{\sl Reading:} Sections #1}
\def\hmk#1#2{\medskip{\sl Problems (due #1): }#2}
%
%       sec macro
%
\def\beginsec#1{
	\bigskip
        \beginsection 
        \par\noindent\centerline{\bf \number\secnumber . #1}
        \medskip
}
\def\endsec{\endsection\par}

\def\beginproblem{
        \advance\probctr by1
        \medbreak\par\noindent
        {\it Problem \number\secnumber .\number\probctr:\/}
}
\def\endproblem{\par\medbreak}

\def\ans{{\medskip\bold Answer: }}

\def\beginsolution{
        \medbreak\par\noindent
        {\it Solution \number\secnumber .\number\probctr:\/}
}
\def\endsolution{\par\medbreak}

\def\beginproblemset{\bigskip\hrule\bigskip\advance\leftskip by 30pt
\advance\rightskip by 30pt\smallfont}
\def\endproblemset{\bigskip\hrule\bigskip\advance\leftskip by -30pt
\advance\rightskip by -30pt\normalfont}
\def\bsp{\beginproblemset\beginproblem}
\def\esp{\endproblem\endproblemset}


%
%	some research note macros
%

\def\beginnote#1{
	%\magnification 1100
	\hsize = 5.9 true in
	\hoffset = 0.45 true in
	\baselineskip = 18pt
        \beginsection 
        \probctr=0
        \par\noindent\centerline{\bf #1}
	\centerline{filename: {\tt\jobname .tex}}
	\centerline{\today}
        \medskip
}
\def\endnote{\endsection\vskip 20pt}


\def\notefontsize{
	\hsize = 5.9 true in
	\hoffset = 0.45 true in
	\baselineskip = 18pt}

%
%       These go at the beginning  of input
%
\global\newtoks\eqrtoks
\global\newtoks\thmtoks
\global\newcount\secnumber
\global\newcount\nonamectr
\global\newcount\probctr



\def\rixend{\closeout\eqroutfile \closeout\thmoutfile \vfill\eject\end}

\message{*** reference macros need to run twice to get references right ***}


==> strongcor.tex <==
\input rixmax
\input epsf
%\draftmode
\def\mcomment#1{}
\font\text=pplr at 10pt
\font\it=pplri at 10pt
\font\bold=phvb at 10pt
%\magnification 1100
        \hsize = 5.9 true in
        \hoffset = 0.45 true in
        \baselineskip = 18pt

%\def\mcomment#1{}
\footline={\hfil}
\footline={\hss\tenrm\folio\hss}
\def\half{{{1}\over{2}}}
\def\hd#1{\bigskip\bigskip{\noindent\bold #1}\par\vrule height\bigskipamount width 0pt\penalty10000}
\def\HB{\overline\HH}
\def\BB{{\Bbb B}}
\def\cd{{\rm cd}}
\def\dist{{\rm dist}}
\def\SH{{\Bbb S\Bbb H}}
\def\twomat#1#2{\left[\matrix{#1\cr #2\cr}\right]}
\def\diag{\mathop{\rm diag}}
\def\qq{{\bf q}}
\def\supp{\mathop{\rm supp}}

\text
\centerline{\bold Absolutely continuous spectrum for a random potential on a tree}
\vskip 10 pt
\centerline{\bold with strong transverse correlations and large weighted loops}
\vskip 20 pt

\centerline{Richard Froese}
\medskip
\centerline{Department of Mathematics}
%\medskip
\centerline{University of British Columbia}
%\medskip
\centerline{Vancouver, British Columbia, Canada}
\bigskip
\centerline{David Hasler}
\medskip
\centerline{Department of Mathematics}
%\medskip
\centerline{The College of William and Mary}
%\medskip
\centerline{Williamsburg, Virginia, USA}
\bigskip
\centerline{Wolfgang Spitzer}
\medskip
\centerline{Institut f\"ur Theoretische Physik}
%\medskip
\centerline{Universit\"at Erlangen-N\"urnberg, Germany}
%\medskip
\centerline{Erlangen, Germany}
\vskip 20pt
\centerline{\today}

\input intro
\input binarytree
\input extensions
\input mubdd
\input meanfield
\input mfbdd
\input refs

\rixend

